Leveraging Wikidata for Geographically Informed Sociocultural Bias Dataset Creation: Application to Latin America

Large Language Models (LLMs) exhibit inequalities with respect to various cultural contexts. Most prominent open-weights models are trained on Global North data and show prejudicial behavior towards other cultures. Moreover, there is a notable lack of resources to detect biases in non-English languages, especially from Latin America (Latam), a continent containing various cultures, even though they share a common cultural ground. We propose to leverage the content of Wikipedia, the structure of the Wikidata knowledge graph, and expert knowledge from social science in order to create a dataset of question/answer (Q/As) pairs, based on the different popular and social cultures of various Latin American countries. We create the LatamQA database of over 26k questions and associated answers extracted from 26k Wikipedia articles, and transformed into multiple-choice questions (MCQ) in Spanish and Portuguese, in turn translated to English. We use this MCQ to quantify the degree of knowledge of various LLMs and find out (i) a discrepancy in performances between the Latam countries, ones being easier than others for the majority of the models, (ii) that the models perform better in their original language, and (iii) that Iberian Spanish culture is better known than Latam one.

==> table_question_examples_small.tex <==
\begin{table*}[h]
\centering
\tiny
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}>{\bfseries}l p{1.98\columnwidth}@{}}
\toprule
\multicolumn{1}{@{}l}{\textbf{Category}} & \textbf{Q \& A} \\
\midrule

FICT & 
% \Q What role did the \textit{Bacab} play in Maya beekeeping? %\\ & 
% \A They were the primary protectors of bees and founders of apiculture. \\

%\addlinespace

& 
\Q What is \textit{glíglico}, and in which literary work does it appear? 
\A \textit{Glíglico} is a fictional language created by Julio Cortázar and appears in his novel \textit{Rayuela}.%, specifically in Chapter 68. 
\\
\midrule

FOOD & 
\Q In which Mexican state is the \textit{memela} considered a traditional dish? 
\A The \textit{memela} is a traditional dish from the state of Puebla. \\


%\addlinespace

& 
\Q What cultural origins does Lima’s \textit{mazamorra morada} have in Peru? 
\A Lima’s \textit{mazamorra morada} has Afro-Peruvian roots and is part of Peru’s culinary identity. \\

\midrule

DIAL & 
\Q What old expression used in Mexico City means “it seems to me” and remains in everyday speech? 
\A The expression “\textit{se me hace}” is used in Mexico City to mean “it seems to me.” \\


%\addlinespace

& 
\Q In Chile, which social group is the term “\textit{flaite}” disparagingly directed toward? 
\A It refers to lower-class individuals who are socially inadapted and aggressive, and also to any vulgar behavior regardless of social origin. \\

\midrule

% 
% .
RELI & 
\Q What is the role of the \textit{machi} in Mapuche culture?
\A The \textit{machi} is a Mapuche medicine central figure, healing physical and spiritual ailments, with religious and social functions \\
%\Q What social function did the Veracruz \textit{fandango} serve in regional cohesion? 
%\A The \textit{fandango} served as a unifying force for the castes living in the region, who did not identify either with peninsular Spaniards or with Indigenous Americans, and called themselves \textit{jarochos}. \\

%\addlinespace

& 
\Q On which day of the month is the tradition of eating \textit{ñoquis} observed in Argentina, Uruguay, Brazil, and Paraguay? \A It is celebrated on the 29th of each month. \\

\midrule

ENTTT & 
\Q According to the article, what is the origin of \textit{cumbia}? 
\A \textit{cumbia} results from a mixture of Indigenous and African influences. \\

%\addlinespace

& 

\Q In which Mexican state is the novel \textit{Falsa liebre} set? 
\A The novel is set in Veracruz, showing the most marginalized and violent side of the region. \\

\bottomrule
\end{tabular}
\caption{Example of questions and answers from different cultural elements.} \label{tab:questions_examples}
\end{table*}



% Performance gaps between Latam Spanish and Portuguese are bigger on the cultural elements containing few example such as "Fictional character" and "Dialect" were the model reach between 75 and 80\% of accuracy.  

%%%%FICT%%%%
% ¿Cómo se relaciona el Caleuche con la identidad cultural del archipiélago de Chiloé?
% A: El Caleuche es un barco fantasma legendario que se vincula a la historia y a las creencias del archipiélago, convirtiéndose en un símbolo central de la mitología chilota.

% Q: ¿Qué papel tenían los bacab en la apicultura maya?
% A: Eran los principales protectores de las abejas y se les consideraba fundadores de la apicultura.

% Q: ¿Qué símbolo de Kukulcán es considerado omnipresente en toda Mesoamérica?
% A: La serpiente emplumada, que representa a Kukulcán, es un símbolo omnipresente en toda Mesoamérica.

% Q: ¿Qué es el glíglico y en qué obra literaria aparece?
% A: El glíglico es una lengua creada por Julio Cortázar y está presente en su novela Rayuela, específicamente en el capítulo 68.


% Q: ¿En qué zonas de Chile es más conocida la leyenda de la Viuda?
% A: En la zona central y sur de Chile.

%%%%FOOD%%%%
% ¿Qué papel tiene el vorí vorí en la identidad cultural de Paraguay?
% Es un elemento distintivo de la gastronomía paraguaya y ha sido reconocido como el caldo de mayor prestigio a nivel mundial en 2023, 2024 y 2025.

% Q: ¿Qué reconocimiento oficial y patrimonial tiene el tereré en Paraguay?
% El tereré es la bebida oficial de Paraguay y, el 17 de diciembre de 2020, la UNESCO lo declaró Patrimonio Cultural Inmaterial de la Humanidad.

% ¿En qué estado de México es la memela considerada un platillo típico?
% La memela es típica del estado de Puebla.

% Q: ¿Qué origen cultural tiene la mazamorra morada limeña en Perú? 
% A: La mazamorra morada limeña tiene influencia afroperuana y forma parte de la identidad culinaria peruana.
% B: La mazamorra morada limeña proviene de la tradición indígena quechua y se conserva como patrimonio gastronómico de los Andes.
% C: Este postre se introdujo en Lima durante la época colonial española, como una adaptación de la mazamorra cordobesa.
% M: Se popularizó a principios del siglo XX, cuando las fábricas de azúcar la promocionaron como acompañamiento de los dulces criollos

% Q: ¿Qué significa la palabra “mbeyú” en guaraní?
% C: Significa ‘torta aplastada’.
% Se traduce como ‘panecillo de queso’, aludiendo a la chipa típica paraguaya.
% Hace referencia al nombre de la fundación de Asunción en el siglo XVI, señalando la ‘ciudad madre’.
% Significa ‘torta de mandioca’, resaltando el ingrediente principal de la preparación.

